Event-Based Signal Temporal Logic Synthesis for Single and Multi-Robot Tasks

We propose a new specification language and control synthesis technique for single and multi-robot high-level tasks; these tasks include timing constraints and reaction to environmental events. Specifically, we define Event-based Signal Temporal Logic (STL) and use it to encode tasks that are reactive to uncontrolled environment events. Our control synthesis approach to Event-based STL tasks combines automata and control barrier functions to produce robot behaviors that satisfy the specification when possible. Our method automatically provides feedback to the user if an Event-based STL task can not be achieved. We demonstrate the effectiveness of the framework through simulations and physical demonstrations of multi-robot tasks.

==> oldBibliography.tex <==
\begin{thebibliography}{99}

\bibitem{baier}Baier, Christel, and Joost-Pieter Katoen. Principles of model checking. MIT press, 2008.
\bibitem{hadas}Kress-Gazit, Hadas, Morteza Lahijanian, and Vasumathi Raman. "Synthesis for robots: Guarantees and feedback for robot behavior." Annual Review of Control, Robotics, and Autonomous Systems 1 (2018): 211-236.
\bibitem{kyriakopoulos}Kyriakopoulos, Savvas G. Loizou Kostas J. "Automatic synthesis of multi-agent motion tasks based on LTL specifications." (2004).
APA	
\bibitem{filippidis}Filippidis, Ioannis, Dimos V. Dimarogonas, and Kostas J. Kyriakopoulos. "Decentralized multi-agent control from local LTL specifications." 2012 IEEE 51st IEEE Conference on Decision and Control (CDC). IEEE, 2012.
APA	
\bibitem{raman1}Raman, Vasumathi, and Hadas Kress-Gazit. "Synthesis for multi-robot controllers with interleaved motion." 2014 IEEE international conference on robotics and automation (ICRA). IEEE, 2014.
APA	
\bibitem{kloetzer}Kloetzer, Marius, and Calin Belta. "Temporal logic planning and control of robotic swarms by hierarchical abstractions." IEEE Transactions on Robotics 23.2 (2007): 320-330.
APA	
\bibitem{chen}Chen, Ji, Salar Moarref, and Hadas Kress-Gazit. "Verifiable control of robotic swarm from high-level specifications." Proceedings of the 17th International Conference on Autonomous Agents and MultiAgent Systems. International Foundation for Autonomous Agents and Multiagent Systems, 2018.
\bibitem{maler}Maler, Oded, and Dejan Nickovic. "Monitoring temporal properties of continuous signals." Formal Techniques, Modelling and Analysis of Timed and Fault-Tolerant Systems. Springer, Berlin, Heidelberg, 2004. 152-166.
\bibitem{raman2}Raman, Vasumathi, et al. "Model predictive control with signal temporal logic specifications." 53rd IEEE Conference on Decision and Control. IEEE, 2014.
\bibitem{zhiyu}Liu, Zhiyu, et al. "Communication-aware motion planning for multi-agent systems from signal temporal logic specifications." 2017 American Control Conference (ACC). IEEE, 2017.
\bibitem{jones}Jones, Austin M., et al. "ScRATCHS: Scalable and Robust Algorithms for Task-based Coordination from High-level Specifications."
\bibitem{reactiveRaman}Raman, Vasumathi, et al. "Reactive synthesis from signal temporal logic specifications." Proceedings of the 18th international conference on hybrid systems: Computation and control. 2015.



\bibitem{donze}Donzé, Alexandre, and Oded Maler. "Robust satisfaction of temporal logic over real-valued signals." International Conference on Formal Modeling and Analysis of Timed Systems. Springer, Berlin, Heidelberg, 2010.
\bibitem{fainekos}Fainekos, Georgios E., and George J. Pappas. "Robustness of temporal logic specifications for continuous-time signals." Theoretical Computer Science 410.42 (2009): 4262-4291.

\bibitem{wieland}Wieland, Peter, and Frank Allgöwer. "Constructive safety using control barrier functions." IFAC Proceedings Volumes 40.12 (2007): 462-467.
\bibitem{ames}Ames, Aaron D., et al. "Control barrier function based quadratic programs for safety critical systems." IEEE Transactions on Automatic Control 62.8 (2016): 3861-3876.
\bibitem{wang}Wang, Li, Aaron D. Ames, and Magnus Egerstedt. "Safety barrier certificates for collisions-free multirobot systems." IEEE Transactions on Robotics 33.3 (2017): 661-674.
\bibitem{lars1}Lindemann, Lars, and Dimos V. Dimarogonas. "Control barrier functions for signal temporal logic tasks." IEEE control systems letters 3.1 (2018): 96-101.
\bibitem{lars2}Lindemann, Lars, and Dimos V. Dimarogonas. "Control Barrier Functions for Multi-Agent Systems Under Conflicting Local Signal Temporal Logic Tasks." IEEE Control Systems Letters 3.3 (2019): 757-762.
\bibitem{lars3}Lindemann, Lars, and Dimos V. Dimarogonas. "Decentralized control barrier functions for coupled multi-agent systems under signal temporal logic tasks." 2019 18th European Control Conference (ECC). IEEE, 2019.
\bibitem{gastin}Gastin, Paul, and Denis Oddoux. "Fast LTL to Büchi automata translation." International Conference on Computer Aided Verification. Springer, Berlin, Heidelberg, 2001.
\bibitem{holzmann}Holzmann, Gerard J. "The model checker SPIN." IEEE Transactions on software engineering 23.5 (1997): 279-295.
\bibitem{duret}Duret-Lutz, Alexandre, et al. "Spot 2.0—A Framework for LTL and $\omega $-Automata Manipulation." International Symposium on Automated Technology for Verification and Analysis. Springer, Cham, 2016.

\end{thebibliography}
